Remote Heart Rate Measurement from Highly Compressed Facial Videos: an End-to-end Deep Learning Solution with Video Enhancement

Remote photoplethysmography (rPPG), which aims at measuring heart activities without any contact, has great potential in many applications (e.g., remote healthcare). Existing rPPG approaches rely on analyzing very fine details of facial videos, which are prone to be affected by video compression. Here we propose a two-stage, end-to-end method using hidden rPPG information enhancement and attention networks, which is the first attempt to counter video compression loss and recover rPPG signals from highly compressed videos. The method includes two parts: 1) a Spatio-Temporal Video Enhancement Network (STVEN) for video enhancement, and 2) an rPPG network (rPPGNet) for rPPG signal recovery. The rPPGNet can work on its own for robust rPPG measurement, and the STVEN network can be added and jointly trained to further boost the performance especially on highly compressed videos. Comprehensive experiments are performed on two benchmark datasets to show that, 1) the proposed method not only achieves superior performance on compressed videos with high-quality videos pair, 2) it also generalizes well on novel data with only compressed videos available, which implies the promising potential for real world applications.

==> new_command.tex <==

%black
\definecolor{bronze}{rgb}{0.8, 0.5, 0.2}
\definecolor{bleudefrance}{rgb}{0.19, 0.55, 0.91}
\definecolor{brown(web)}{rgb}{0.65, 0.16, 0.16}
\definecolor{cadmiumorange}{rgb}{0.93, 0.53, 0.18}
%for Zitong Yu
\newcommand\Yu[1]{\textcolor{cadmiumorange}{#1}}

%for Wei Peng
\newcommand\pw[1]{\textcolor{bleudefrance}{#1}}
\newcommand\pwC[1]{\textcolor{bleudefrance}{[Wei Peng: #1]}}
%for Xiaobai Li
\newcommand\Li[1]{\textcolor{green}{#1}}

%for Xiaopeng Hong
\newcommand\XP[1]{\textcolor{red}{#1}}
\newcommand\XPC[1]{\textcolor{red}{[Xiaopeng: #1]}}

\newcommand\XPCC[2]{\textcolor{red}{\textit{[Xiaopeng: #1]}\textbf[#2]}}

\newcommand\XPDel[1]{\textcolor{red}{\sout{{#1}}}}

%for Guoying Zhao
\newcommand\Zhao[1]{\textcolor{brown(web)}{#1}}

%updating
\newcommand\up[1]{\textcolor{gray}{#1}}

\def\eg{\emph{e.g.}} \def\Eg{\emph{E.g.}}
\def\ie{\emph{i.e.}}
\def\Ie{\emph{I.e.}}
\def\cf{\emph{c.f.}} \def\Cf{\emph{C.f.}}
\def\etc{\emph{etc.}} \def\vs{\emph{vs.}}
\def\wrt{w.r.t.} 
\def\dof{d.o.f.}
\def\etal{\emph{et al.}}
\def\aka{\emph{a.k.a.}}
